GPT Store Mining and Analysis

As a pivotal extension of the renowned ChatGPT, the GPT Store serves as a dynamic marketplace for various Generative Pre-trained Transformer (GPT) models, shaping the frontier of conversational AI. This paper presents an in-depth measurement study of the GPT Store, with a focus on the categorization of GPTs by topic, factors influencing GPT popularity, and the potential security risks. Our investigation starts with assessing the categorization of GPTs in the GPT Store, analyzing how they are organized by topics, and evaluating the effectiveness of the classification system. We then examine the factors that affect the popularity of specific GPTs, looking into user preferences, algorithmic influences, and market trends. Finally, the study delves into the security risks of the GPT Store, identifying potential threats and evaluating the robustness of existing security measures. This study offers a detailed overview of the GPT Store's current state, shedding light on its operational dynamics and user interaction patterns. Our findings aim to enhance understanding of the GPT ecosystem, providing valuable insights for future research, development, and policy-making in generative AI.

==> sections/limitation.tex <==
\section{Threats to Validity}
In our study of the factors influencing featured GPTs, the limited number of samples available might have introduced selection bias, meaning the samples chosen may not represent all types of GPTs in the GPT Store. This bias could affect our understanding of which factors truly influence the popularity of GPTs, thereby impacting the generalizability and accuracy of our research findings. Moreover, in assessing the security risks of the GPT Store, time and technical constraints prevented us from conducting large-scale systematic tests; instead, we relied on sampling tests. Although this approach provided some insight into security risks, it may not have revealed all potential threats comprehensively.  These limitations indicate that future research should expand the sample size, improve data collection methods, and conduct more in-depth security testing to enhance the reliability and applicability of the research outcomes.
\label{Sec:limitations}

